Fungi: Typed incremental computation with names

Incremental computations attempt to exploit input similarities over time, reusing work that is unaffected by input changes. To maximize this reuse in a general-purpose programming setting, programmers need a mechanism to identify dynamic allocations (of data and subcomputations) that correspond over time. We present Fungi, a typed functional language for incremental computation with names. Unlike prior general-purpose languages for incremental computing, Fungi's notion of names is formal, general, and statically verifiable. Fungi's type-and-effect system permits the programmer to encode (program-specific) local invariants about names, and to use these invariants to establish global uniqueness for their composed programs, the property of using names correctly. We prove that well-typed Fungi programs respect global uniqueness. We derive a bidirectional version of the type and effect system, and we have implemented a prototype of Fungi in Rust. We apply Fungi to a library of incremental collections, showing that it is expressive in practice.

==> Makefile <==
.PHONY: submit figs fast

submit : figs
	pdflatex fungi-lang
	bibtex fungi-lang || true
	pdflatex fungi-lang
	pdflatex fungi-lang
	mkdir submitted 2> /dev/null || true
	mv fungi-lang.pdf submitted/supp.pdf
	pdflatex '\def\MainOnly{1} \input{fungi-lang.tex}'
	mv fungi-lang.pdf submitted/main.pdf
	./assemble-anon-supp

figs:
	pdflatex icintro.tex
	pdflatex dedup_3439.tex
	pdflatex dedup_1439.tex
	pdflatex dedup_1439_from_3439.tex
	pdflatex dedup_x4x.tex	

fast:
	pdflatex fungi-lang

fast-figs: figs fast

main:
	pdflatex '\def\MainOnly{1} \input{fungi-lang.tex}'



==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

We use our core calculus type system from \Secref{sec:typesystem} as
the basis for a \emph{family} of core calculi for reasoning about
programs use caches with explicit names.

In particular, we discuss an extension for typing a mixture of
incremental and functional reactive programming.

\subsection{Functional reactive programming with explicit names.}

Functional reactive programming (FRP) models provide abstractions
for describing time-varying behavior, often using high-level
abstractions for streams and/or events.
%
Behind the scenes, a \emph{reactive loop} executes as the main thread
of control, re-executing code from the FRP program as time advances.
%
Based on \Secref{sec:typesystem}, we sketch a core calculus where these
reactive loops' bodies may be incorporated into a an incremental
program with change propagation.

\paragraph{Proposed static semantics.}
%
To statically approximate the effects of reactive loops, we propose
augmenting our notion of effects (tracking reads and writes,
\emph{now}) to additionally mark where \emph{delayed feedback effects}
occur, allowing programmers to combine such loops and general-purpose
incremental computing.
%
Now effects consist of triples~$<<R;W;F>>$ where name sets $R$, $W$
and $F$ give the read, write and nominal feedback sets, respectively.

To control nominal feedback, we propose the following two primitives:
%
\[
\Infer{delay}
{\Gamma |- v : \Nm[[X]] \\ \Gamma |- e : E }
{\Gamma |- \keyword{delay}(v,e) : \F \big( \Thk{X}{E} \big) |> <<\emptyset; \emptyset; X>> }
~~
\Infer{loop}
{\arrayenvbl{ \Gamma |- e_1 : A |> <<R; W; F>> \\ \Gamma |- e_2 : \textsf{Loop}~A |> <<R{\disj}F; W; F>>} }
{\Gamma |- \keyword{loop}(e_1,e_2) : \F A |> <<R{\disj}W{\disj}F; W{\disj}F; \emptyset>>}
\]
%
The statics of the delay rule says that we can name a \emph{delayed}
thunk; the dynamic semantics of this primitive, discussed more below,
is to write this name (drawn from~$X$) with expression~$e$ \emph{just before the next
  loop iteration}.
%
(For simplicity here, we omit the write scope monad that is present in
the \Secref{sec:typesystem} rules; this can be easily added).
%
In the conclusion of the rule, we treat the loop's ``feedback writes''
like ordinary writes.
%
Within the loop, \code{let}-sequencing delayed writes works
analogously to ordinary writes: one cannot delay the same name twice.
Further, to restrict store updates to the loop iteration boundaries,
we do not permit the program to write and to also delay the same name.

To define loops, the programmer provides two expressions:
expression~$e_1$ creates the initial feedback state, performing
reads~$R$, writes~$W$ and delayed writes~$F$.  Expression~$e_2$ may
assume that $F$ has been written, and may read from it; by contrast,
the rule ``rewinds'' the write set~$W$, by \emph{not} assuming that it
has been written for $e_2$, which may re-perform these writes~$W$
(incrementally-updating prior allocations, like the \emph{editor}
would), and in the process, it may update (``re-delay'') thunks in~$F$
for the next loop iteration.

That sub-expression~$e_2$ has type $\textsf{Loop}~A |> \e$, which is a
computation that produces the following (recursive) sum type:
%
\[
\big(
  \textsf{Loop}~A |> \e
\big)
= 
\big(
  \F (A + \Thk{X}{(\textsf{Loop}_X~A) |> \e}) |> \e
\big)
\]
%
Statically, the expression $e_2$ will either produce a value of
type~$A$, or a thunk that produces more thunks (and perhaps possibly a
value) in the future.

\paragraph{Proposed dynamic semantics.}
The dynamic semantics of loops consist of re-running expression~$e_2$
until it produces its value (if ever) and in so doing, the write and
delay effects of expression~$e_2$ will typically \emph{overwrite} the
previous reads of $e_2$, creating an incrementalized feedback loop,
whose execution is guided by change propagation.

As mentioned above, the dynamic semantics treats delayed writes
specially, by delaying them until the \textsf{Loop} fully completes an
iteration.
%
This proposal corresponds closely with prior work on synchronous,
discrete-time FRP---especially~\citet{Krishnaswami13}.
%
A key difference is that in our programming model, we mix incremental
and reactive computations, and in both cases, names are explicitly
provided by the programmer.


==> fig-expr.tex <==
\begin{figure}[htbp]
  \centering
 
\begin{grammar}
  Values
  & $v$
      &$\bnfas$&
      $x$
      \\ &&& $\bnfaltbrk \unitexp$ & 
      \\ &&& $\bnfaltbrk \Pair{v_1}{v_2}$ & introduce product
      \\ &&& $\bnfaltbrk \inj{i}{v}$ & introduce sum
      \\ &&& $\bnfaltbrk \name{M}$ & the name $n$, as a value
      \\ &&& $\bnfaltbrk \namefn{M}$ & the name term $M$
      \\ &&& $\bnfaltbrk \refv{M}$ & ref cell at location $n$
      \\ &&& $\bnfaltbrk \thunk{M}$ & thunk at location $n$
%      \\ &&& $\bnfaltbrk \unthunk{n}$ &
  \\[1ex]
  Terminal expressions
  & $t$
      &$\bnfas$&
              $\Ret{v}$ & return the value $v$
      \\ &&& $\bnfaltbrk \lam{x} e$ & ordinary $\lambda$
  \\[1ex]
  Expressions
  & $e$
      &$\bnfas$&
           $t$ & terminal expression (above)
      \\ &&& $\bnfaltbrk \Split{v}{x_1}{x_2}{e}$ & eliminate product
      \\ &&& $\bnfaltbrk \Case{v}{x_1}{e_1}{x_2}{e_2}$ & eliminate sum
%      \\ &&& $\bnfaltbrk \Ret{v}$ & return the value $v$
%      \\ &&& $\bnfaltbrk \lam{x} e$ & ordinary $\lambda$
      \\ &&& $\bnfaltbrk \Let{e_1}{x}{e_2}$ &
      \\ &&& $\bnfaltbrk e\;v$ & ordinary function application
      \\ &&& $\bnfaltbrk \Refe{v} v$ & allocate a ref cell
      \\ &&& $\bnfaltbrk \Thunk{v} e$ & create a thunk
%      \\ &&& $\bnfaltbrk \Unthunk{v}$ &
      \\ &&& $\bnfaltbrk \Force{v}$ & force a thunk
      \\ &&& $\bnfaltbrk \Get{v}$ & get the contents of a ref cell
%      \\ &&& $\bnfaltbrk \Ns{v}{e}$ &
      \\ &&& $\bnfaltbrk \Scope{M}{e}$ & enter a namespace
      \\ &&& $\bnfaltbrk v_1\;v_2$ & name function $v_1$ applied to name $v_2$
%      \\ &&& $\bnfaltbrk \namearrintro{a}{e}$ & intro.\ form for $\Namearrsym$
%      \\ &&& $\bnfaltbrk \namearrelim{e}{t}$ & elim.\ form for $\Namearrsym$
\end{grammar}

  \caption{Syntax of expressions}
  \label{fig:expr}
\end{figure}


% Local Variables:
% mode: latex
% TeX-master: "types"
% End:


==> fig-inc-dynamics.tex <==
\begin{figure}[thbp]

\begin{grammar}
Graphs 
& $G$,$H$
    & $\bnfas$ & $\cdots$
\\ &&& $\bnfaltbrk$ $G, p {:} ( e , t )\,{@}\,M$ & $p$ points to thunk $e$ in namespace $M$ with cached result $t$
\\ &&& $\bnfaltbrk$ $G, (p, a, b, q)$ & $p$ depends on $q$ due to action $a$ with status $b$

\\[1ex]

Edge actions
& $a$ 
  & $\bnfas$ & &
   \text{For edge $(p, a, b, q)$, the computation at $p$\dots}
\\ &&&              $\textsf{alloc} \, v$ & $\dots$ created reference $v$ at $q$
\\ &&& $\bnfaltbrk$ $\textsf{alloc} \, e$ & $\dots$ created thunk $e$ at $q$
\\ &&& $\bnfaltbrk$ $\textsf{obs} \, v  $ & $\dots$ read $q$'s value, which was $v$
\\ &&& $\bnfaltbrk$ $\textsf{obs} \, e  $ & $\dots$ forced thunk $q$, which normalized as $e$

\\[1ex]

Edge statuses
& $b$ 
  & \bnfas 
     & \textsf{clean} 
     & value or computation at sink is out of date
\\ &&& $\bnfaltbrk$ \textsf{dirty} 
     & value or computation at sink is up to date
\end{grammar}

\caption{Graphs with structure for incremental computation: cached results and dependency edges}
\label{fig:graph-incremental}
\end{figure}

\begin{figure}[htbp]
  \centering

  %% \judgbox
  %%     {e \terminal}
  %%     {Expression $e$ is terminal}
  %% \vspace{-2ex}
  %% \begin{mathpar}
  %%   \Infer{}
  %%       {}
  %%       {\Ret{v} \terminal}
  %%   \and
  %%   \Infer{}
  %%       {}
  %%       {(\lam{x} e) \terminal}
  %%   \and
  %%   \Infer{}
  %%       {}
  %%       {(\namearrintro{a}{e}) \terminal}
  %% \end{mathpar}
  
  \judgbox{\PreSt{G_1}{M}{m} e !! G_2 ; e'}{
    Under graph $G_1$, namespace $M$ and current node $m$, 
    $e$ produces $G_2$ and $e'$.}
\begin{mathpar}\end{mathpar}
\\[-7mm]
\colorbox{light-gray}{
  \begin{mathpar}
    \small
    \Infer{thunk-clean}
      {
        (M\,p) \nteval q
        \\
        \textsf{exp}(G, q) = e
        \\
        \textsf{ns}(G, q) = M
      }
      {
        \PreSt{G} {M}{m} \Thunk{\name{p}} e !! 
        G, (m,\textsf{alloc}\,e,\textsf{clean},q); \Ret{\thunk{q}}
      }
    \and
    \Infer{thunk-dirty}
      {
        (M\,p) \nteval q
        \\ 
        G_1\{q{\mapsto}e\,{@}\,M\} = G_2
        \\
        \textsf{dirty-paths-in}(G_2, q) = G_3 
      }
      {
        \PreSt{G_1} {M}{m} \Thunk{\name{p}} e !! 
        G_3, (m,\textsf{alloc}\,e,\textsf{clean},q); \Ret{\thunk{q}}
      }
    \and
    \Infer{ref-clean}
        {
          (M\,p) \nteval q
          \\ 
          G(q) = v
        }
        {
          \PreSt{G} {M}{m} \Refe{\name{p}}{v} !! 
          G, (m,\textsf{alloc}\,v,\textsf{clean},q); \Ret{\refv{q}}
        }
    \and
    \Infer{ref-dirty}
        {
          (M\,p) \nteval q
          \\ 
          G_1\{p{\mapsto}v\} = G_2 
          \\ 
          \textsf{dirty-paths-in}(G_2, p) = G_3 
        }
        {
          \PreSt{G_1} {M}{m} \Refe{\name{p}}{v} !! 
          G_3, (m,\textsf{alloc}\,v,\textsf{clean},q); \Ret{\refv{q}}
        }
    \and
    \Infer{force-clean}
        {
          G_1 |- p *> G_2 ; t
%          \\
%          G_2(p) = (e, t)\,{@}\,m_0
        }
        {
          \PreSt{G_1} {M}{m} \Force{\thunk{p}} !! 
          G_2, (m,\textsf{obs}\,t,\textsf{clean},p); t
        }
    \and
    \Infer{get-clean}
      { G(q) = v }
      { \PreSt{G} {M}{m} \Get{\refv{q}} !! 
        G, (m,\textsf{obs}\,v,\textsf{clean},q); \Ret{v} }
  \end{mathpar}
  }
  \caption{Incremental evaluation rules: Ref and thunk reuse guided by dirtying and cleaning the DCG.}
  \label{fig:dynamics-incremental}
  \label{fig:inc-dynamics}

\vspace*{5mm}

 \judgbox{G_1 |- p *> G_2 ; t}{
    Under graph $G_1$, cleaning the DCG rooted at node $p$ produces $G_2$ and $t$.}

\begin{mathpar}
    \Infer{clean-done}
        {
          \textsf{all-clean-out}(G, p)
          \\\\
          G(p) = (e, t)\,{@}\,M
        }
        {
          G |- p *> G; t
        }
    \and
    \Infer{clean-edge}
      {
        \arrayenvbl{
          \textsf{all-clean-out}((G_1, G_2), q_2)
          \\
          \textsf{consistent-action}((G_1, G_2), a, q_2)
          \\
          G_1, (q_1, a, \textsf{clean}, q_2), G_2 |- p *> G_3; t
        }
      }
      {
        G_1, (q_1, a, \textsf{dirty}, q_2), G_2 |- p *> G_3; t
      }
    \and
    \Infer{clean-node}
      {
        \arrayenvbl{
          \big(\textsf{exp}(G_1, q) = e\big)
          \wedge
          \big(\textsf{ns}(G_1, q) = M\big)
          \\
          \textsf{del-edges-out}(G_1\{q \mapsto e\,{@}\,M\}, q) = G_1'
          \\
          \D :: \PreSt{G_1'}{M}{q} e !! G_2; t
          \\
          \Cc :: G_2\{q \mapsto (e, t)\} |- p *> G_3, t'
          \\
          \DHasEffects{\D}{R_\D}{W_\D} \Rightarrow \big(
            (\DHasEffects{\Cc}{R_\Cc}{W_\Cc})
            \wedge
            (W_\D \disjoint W_\Cc)
            \wedge
            (R_\D \disjoint W_\Cc)
          \big)
        }
      }
      {
        G_1 |- p *> G_3; t'
      }
\end{mathpar}

  \caption{Incremental cleaning rules: Cleaning graph nodes and edges.}
  \label{fig:dynamics-clean}

\end{figure}


==> fig-index-eval.tex <==
\begin{figure}
  \judgbox{i \Value}
          {Index $i$ is a value (it evaluates to itself)}
\begin{mathpar}
\Infer{val-singleton}
{ }
{ \{ N \} \Value }
%
~~~
\Infer{val-disj}
{ i \Value 
  \\
  j \Value 
}
{ i \disj j \Value }
%
~~~
\Infer{val-pair}
{ i \Value 
  \and
  j \Value 
}
{ \Pair{i}{j} \Value }
%
~~~
\Infer{val-abs}
{ }
{ \lam{a}{i} \Value }
\end{mathpar}

\vspace{1ex}

\judgbox{i !! j}
        {Index~$i$ evaluates to index~$j$}
\vspace{-2ex}
\begin{mathpar}
\Infer{\!value}
    {i \Value}
    { i !! i }
~~~~
\Infer{\!pair}
    {
      i_1 !! j_1
      ~~~~
      i_2 !! j_2
    }
    {\Pair{i_1}{i_2} !! \Pair{j_1}{j_2}}
~~~~
\Infer{\!proj}
    { i !! \Pair{j_1}{j_2} }
    { \Proj{b}{i} !! j_b}
% \and
% \Infer{\!proj2}
% { i !! (j_1, j_2) }
% { \Proj{2}{i} !! j_2}
~~~~
\Infer{\!union}
    {
      \arrayenvbl{
        i !! i' 
        \\
        j !! j'
      }
    }
    {(i \union j) !! (i' \union j')}
\and
\Infer{\!disj}
    {
      \arrayenvbl{
        i !! i' 
        \\
        j !! j'
      }
      ~~~~~
      ||- i' \disj j' : \namesetsort
    }
    {(i \disj j) !! (i' \disj j')}
\and
\Infer{\!app}
{ i !! \lam{a}{i'}
\\
j !! j'
\\
[j'/a] i' !! k
}
{i(j) !! k}
\and
\Infer{\!map-set}
{ j !! j' 
  \\
\mapset{M}{j'}{j''} 
}
{ M [[ j ]] !! j'' }
\end{mathpar}

\judgbox{ \mapset{M}{X}{Y} }
        {Name term function $M$, applied to each member of $X$, yields name set $Y$}
\begin{mathpar}
\Infer{Single}
{ M ( N ) \nteval V }
{ \mapset{M}{ \{ N \} }{ \{ V \} } }
\and
\Infer{Apart}
{ \mapset{ M }{ X_1 }{ Y_1 } 
  \\
  \mapset{ M }{ X_2 }{ Y_2 } 
}
{ \mapset{ M }{ X_1 \disj X_2 }{ Y_1 \disj Y_2 } }
\vspace*{-1.5ex}
\end{mathpar}

\caption{Evaluation rules for indices}
\label{fig:index-eval}
\end{figure}


% Local Variables:
% TeX-master: "typed-adapton"
% End:


==> fig-namestep.tex <==



\THIS\FIGURE\IS\OBSOLETE



\begin{figure}[t]
  \centering

  \begin{grammar}
      Name term values
     &$\Mv$
          &$\bnfas$&
          $n
          \bnfalt \lam{a} M
          \bnfalt a
          \bnfalt \unitexp
          \bnfalt \Pair{\Mv}{\Mv}
          \bnfalt \Mv.1
          \bnfalt \Mv.2
          $
  \end{grammar}

  \judgbox{M \nteval \Mv}
          {Name term $M$ evaluates to name term value $\Mv$
          }
  \begin{mathpar}
    \Infer{teval-value}  % name, abstraction, [variable], unit
       {}
       {\Mv \nteval \Mv}
    \and
    \Infer{teval-app}
        {
          M_1 \nteval \lam{a} M
          \\
          M_2 \nteval \Mv_2
          \\
          [\Mv_2 / a]M \nteval \Mv
        }
        {(M_1\,M_2) \nteval \Mv}
    \and
    \Infer{teval-pair}
        {
          M_1 \nteval \Mv_1
          \\
          M_2 \nteval \Mv_2
        }
        {
          \Pair{M_1}{M_2} \nteval \Pair{\Mv_1}{\Mv_2}
        }
    \and    
    \Infer{teval-append}
        {
          M \nteval \Mv
        }
        {
          \arrayenvbl{
            M.1 \nteval \Mv.1
            \\
            M.2 \nteval \Mv.2
          }
        }     
  \vspace*{-2ex}
  \end{mathpar}

  \caption{Name term evaluation}
  \label{fig:namestep}
\end{figure}


% Local Variables:
% TeX-master: "types"
% End:


==> fig-syntax-types-compact.tex <==
\begin{figure}[t]
  \centering
 
\begin{grammar}
  Name terms
 &$M$
      &$\bnfas$&
      $n 
\bnfalt \unitexp
 \bnfalt \lam{a} M
 \bnfalt a
 \bnfalt \idxapp{M}{M}
 \bnfalt M.1
 \bnfalt M.2
 \bnfalt \Pair{M_1}{M_2}
$
  \\[0.6ex]
  Index sorts
  & $\sort$
      &$\bnfas$&
      $\namesort
   \bnfalt \namesetsort
   \bnfalt \unitsort
   \bnfalt \sort * \sort
   \bnfalt \sort @> \sort$
  \\[0.6ex]
%   Symbols
%   & $s$
%   \\[0.6ex]
  Names
  & $n, m, p, q$
     &$\bnfas$&
$ \rootname
   \bnfalt n.1 \bnfalt n.2
   \bnfalt \Pair{n_1}{n_2}$
  \\[0.6ex]
  Index variables
  & $a$
  \\
  Index exprs.
  & $i, X, Y, Z, R, W$
      &$\bnfas$&
      $a
 \bnfalt \{n\}
 \bnfalt X \disj Y
 \bnfalt \unitindex
      \bnfalt \Pair{i}{i}
      \bnfalt M[[i]]
      $
\end{grammar}
\lesscaptionspace

  \caption{Syntax of indices, including names}
  \label{fig:syntax-indices}
\end{figure}



\begin{figure}[htbp]
  \centering
 
\begin{grammar}
  Kinds
  & $K$
      &$\bnfas$&
      $\type
      \bnfalt \type => K
      \bnfalt \sort => K
      $
%   \\[0.6ex]
%   Propositions
%   & $P$
%       &$\bnfas$&
%       $
%       \trueprop
%       \bnfaltBRK P \andprop P
%       \bnfaltBRK X \disj Y
%       \bnfaltBRK X \subseteq Y
%       $
  \\[0.6ex]
  Effects
  & $\e$
      &$\bnfas$&
               $<<W; R>>$
  \\[0.6ex]
  Type constructors
  & $d$
  \\
  Type variables
  & $\alpha$
  \\
  Value types
  & $A, B$
      &$\bnfas$&
            $\alpha
      \bnfalt d
      \bnfalt A + B
      \bnfalt  A ** B
      \bnfalt  \Unit
      \bnfalt \Ref{i}{A}
      \bnfalt \Thk{i}{E}
%      \bnfalt \Unthk{i}{E}$  & named ``unthunk'' (no effects) % unthunk
      \bnfaltBRK  A[[i]]
      \bnfalt  A\;B
      \bnfalt  \Name{i}
      \bnfalt  (\namesort @> \namesort)[[M]]$
  \\[0.6ex]
  Computation types
  & $C, D$
      &$\bnfas$&
      $\F A
 \bnfalt A -> E$
  \\[0.6ex]
  \dots with effects
  & $E$
      &$\bnfas$&
      $C |> \e
 \bnfalt \All{\alpha : K} E
% % \bnfalt \Univ{a : \sort} E  $   & index polymorphism
 \bnfalt \All{a : \sort} E  $
% % \bnfalt \Namearr{a}{\sort} E$   & name function polymorphism
%  \bnfalt P --> E  $   & guarded type
 \\[0.6ex]
  Typing contexts
  & $\Gamma$
    &$\bnfas$&
    $\cdot
  \bnfalt \Gamma, p : A
  \bnfalt \Gamma, p : E
  \bnfalt \Gamma, x : A$
%  \bnfalt \Gamma, P$ & truth of proposition
\end{grammar}
\lesscaptionspace

  \caption{Syntax of kinds, effects and types}
  \label{fig:syntax-types}
\end{figure}


% Local Variables:
% mode: latex
% TeX-master: "typed-adapton"
% End:


==> meta-dynamics.tex <==
\section{Dynamics Metatheory: From-Scratch Consistency}
\Label{apx:metatheory}

\subsection{Overview}

Our main formal result in this paper, \emph{from-scratch consistency},
states that given an evaluation derivation
corresponding to an incremental computation, we can construct a derivation
corresponding to a non-incremental computation that returns the same result
and a corresponding graph.  That is, the incremental computation is consistent
with a computation in the simpler non-incremental system.

To properly state the consistency result, we need to define what it means for a graph to
be well-formed (\Sectionref{sec:graph-wf}),
%
relate the incremental computation's DCG
to the non-incremental computation's store (\Sectionref{sec:restriction}),
describe the sets of nodes read and written by an evaluation derivation
(\Sectionref{sec:rw-sets}),
and prove a store weakening lemma~(\Sectionref{sec:weakening}).
The consistency result itself is stated and proved in \Sectionref{sec:fsc}.



\subsection{Graph Well-Formedness}
\Label{sec:graph-wf}

\begin{figure*}
\small
%\ottdefnsGrwf
\begin{mathpar}
\Infer{Grwf-emp}
    { }
    {G |- \cdot \wf}
\and
\Infer{Grwf-ref}
    {G |- H \wf
    \\
    G(p) = v
    }
    {G |- H, p:v \wf}
\and
\Infer{Grwf-thunk}
    {G |- H \wf
    \\
    G(p) = e
    }
    {G |- H, p:e \wf}
\and
\Infer{Grwf-thunkCache}
    {
      G |- H \wf
      \\
      \arrayenvbl{
        G(p) = (e,e')
        \\
        \textsf{if}~\textsf{all-clean-out}(G,p)~\textsf{then}~\D \derives \PreSt{G}{p}{w} e !! G ; e'
        \\
        \textsf{if not}~\textsf{all-clean-out}(G, p)~\textsf{then}~\textsf{all-dirty-in}(G, p)
      }
    }
    {G |- H, p:(e,e') \wf}
\and
\Infer{Grwf-dirtyEdge}
    {
    G |- H \wf
    \\
    (p, a, \textsf{dirty}, q) \in G
    \\
    q \in \textsf{dom}(H)
    \\
    \textsf{if}~(p_0, a_0, b_0, p) \in G~\textsf{then}~b0 = \textsf{dirty}
    }
    {G |- H, (p, a, \textsf{dirty}, q) \wf}
\and
\Infer{Grwf-cleanEdge}
    {
    G |- H \wf
    \\
    (p, a, \textsf{clean}, q) \in G
    \\
    \textsf{consistent-action}(H, a, q)
    \\
    \textsf{all-clean-out}(G, q)
    }
    {G |- H, (p, a, \textsf{clean}, q) \wf}
\end{mathpar}
\vspace{-3ex}
\caption{Graph well-formedness rules}
\FLabel{fig:graph-wf}
\end{figure*}

The judgment $G |- H \wf$ is read ``$H$ is a well-formed subset of $G$''.
It implies that $H$ is a linearization of a subset of $G$: within $H$,
information sources appear to the left of information sinks,
dependency edges point to the left, and information flows to the right.
Consequently, $H$ is a dag.

For brevity, we write $G \wf$ for $G |- G \wf$, threading
the entire graph $G$ through the rules deriving $G |- H \wf$.
The well-formedness rules in \Figureref{fig:graph-wf} decompose the right-hand
graph, and work as follows:

\begin{itemize}
\item
  For values (Grwf-val) and thunks with no cached result (Grwf-thunk),
  the rules only check the correspondence between $G$ (the entire graph)
  and $H$ (the subgraph).

\item For thunks with a cached result, Grwf-thunkCache
  examines the outgoing edges.  If they are all clean, then it checks
  that evaluating $e$ \emph{again}
  would not change the graph at all: $\D \derives \PreSt{G}{p}{w} e !! G ; t$.
%  (It also checks that the derivation $\D$ is ``satisfactory''; see
%  \Sectionref{sec:satisfactory-derivations}.)
  If one or more edges are dirty, it checks that all incoming edges are dirty.

\item
  Grwf-dirtyEdge checks that
  all edges flowing into a dirty edge are dirty:
  given edges from $p$ to $q$ and from $q$ to $r$, where
  the edge from $q$ to $r$ is dirty (meaning that $q$ depends on $r$ and $r$ needs
  to be recomputed), the edge from $p$ to $q$ should
  also be dirty.  Otherwise, we would think we could reuse the result in $p$,
  even though $p$ (transitively) depends on $r$.

  Conversely, if an edge from $p$ to $q$ is clean (Grwf-cleanEdge),
  then all edges out from $q$ must
  be clean (otherwise we would contradict the ``transitive dirtiness'' just described).
  Moreover, the action $a$ stored in the edge from $p$ to $q$ must be consistent
  with the contents of $q$.
\end{itemize}


\subsection{From Graphs to Stores: the Restriction Function}
\Label{sec:restriction}

To relate the graph associated with an incremental evaluation to
the store associated with a non-incremental evaluation, we define
a function~$\restrict{G}{P}$ that restricts $G$ to a set of pointers
$P$, drops cached thunk results (*), and erases all edges (**):
%
\begin{defn}[Restriction]
\Label{def:restrict}
\[
  \begin{array}{cr@{~~}c@{~~}lll}
    &\restrict{\emptyset}{P} &=& \emptyset
    \\[1ex]
    &\restrict{G, p:v}{P} &=& \restrict{G}{P}, p:v & \text{if $p \in P$}
    \\
    &\restrict{G, p:v}{P} &=& \restrict{G}{P} & \text{if $p \notin P$}
    \\[1ex]
    &\restrict{G, p:e}{P} &=& \restrict{G}{P}, p:e & \text{if $p \in P$}
    \\
    &\restrict{G, p:e}{P} &=& \restrict{G}{P} & \text{if $p \notin P$}
    \\
    \text{(*)}&\restrict{G, p:(e,t)}{P} &=& \restrict{G}{P}, p:e & \text{if $p \in P$}
    \\
    &\restrict{G, p:(e,t)}{P} &=& \restrict{G}{P} & \text{if $p \notin P$}
    \\[1ex]
    \text{(**)}&\restrict{G, (p,a,b,q)}{P} &=& \restrict{G}{P}
  \end{array}
\]
\end{defn}



\paragraph{Agreement.}  We want to express a result
 (\Lemmaref{lem:respect-write}) that evaluation only affects pointers in the write set
$W$, leaving the contents of other pointers alone, so we define what it means
to leave pointers alone:

\begin{defn}[Agreement on a pointer]
  Graphs $G_1$ and $G_2$ \emph{agree on}
  $p$ iff either $G_1(p) = G_2(p)$,
  or $p:v \in G_1$ and $p:v \in G_2$.
\end{defn}

\begin{defn}[Agreement on a set of pointers]
  Graphs $G_1$ and $G_2$ \emph{agree on}
  a set $P$ of pointers iff $G_1$ and $G_2$
  agree on each $p \in P$.
\end{defn}

\begin{lem}[Respect for write-set]
\Label{lem:respect-write}
~\\
   If $\D \derives \PreSt{G}{p}{w} e !! G';t$ where $\D$ is incremental
%   \\
   and $\DHasEffects{\D}{R}{W}$
%   \\
%   and $\D \monotonic$
   \\
   then $G'$ agrees with $G$ on $\dom{G} - \dom{W}$.
\end{lem}
\begin{proof}
  By a straightforward induction on $\D$, referring to \Definitionref{def:rw}.

  In the Eval-forceClean case, use the fact that $G'$ differs
  from $G$ only in the addition of an edge, which does not affect agreement.
\end{proof}


\subsection{Satisfactory derivations}
\Label{sec:satisfactory-derivations}

In our main result~(\Theoremref{thm:fsc}), we will assume that all input
and output graphs appearing within a derivation are well-formed,
and that the read- and write-sets are defined:

\begin{defn}[Locally satisfactory]
\Label{def:local-sat}
~\\
     A derivation
     $\D \derives \PreSt{G_1}{p}{w} e !! G_2 ; t$
     is \emph{locally satisfactory}
     if and only if

     \begin{enumerate}[(1)]
     %
    \item  % (1)
           $G_1 \wf$ and $G_2 \wf$

     \item  % (2) ``functional''
           $\DHasEffects{\D}{R}{W}$ is defined

     \end{enumerate}
\end{defn}

\begin{defn}[Globally satisfactory]
\Label{def:global-sat}
~\\
    An evaluation derivation
    $\D \derives \PreSt{H_1}{p}{w} e !! H_2 ; t$
    is \emph{globally satisfactory}, written~$\D \satisfactory$,
    if and only if
    $\D$ is locally satisfactory
    and all its subderivations are locally satisfactory.
\end{defn}


\subsection{Weakening}
\Label{sec:weakening}

The main result needs to construct a non-incremental derivation
in a different order from the given incremental derivation.
In particular, the first evaluation $\D_1$ done in Eval-computeDep
will be done ``later'' in the non-incremental derivation.
Since it
is done later, the graph may have new material $G'$,
and we need a weakening lemma to move from a non-incremental
evaluation of $\D_1$ (obtained through the induction hypothesis)
to a non-incremental evaluation over the larger graph.

\begin{lem}[Weakening (non-incremental)]
\Label{lem:weakening-ni}
~\\
   If $\D \derives \PreSt{G_1}{p}{w} e !! G_2; t$
   and $\D$ is non-incremental
   \\
   and $G'$ is disjoint from $G_1$ and $G_2$
   \\
   then $\D' \derives \PreSt{G_1, G'}{p}{w} e !! G_2, G'; t$
   where $\D'$ is non-incremental.
\end{lem}
\begin{proof}
  By induction on $\D$.

  \begin{itemize}
      \ProofCasesRules{Eval-term, Eval-app, Eval-fix, Eval-bind,
                       Eval-case, Eval-split, Eval-fork, Eval-namespace, Eval-nest}

          These rules do not manipulate the graph, so
          just use the i.h.\ on each subderivation, then apply the same rule.

      \ProofCaseRule{Eval-refPlain}
           Since $\update{G_1}{q}{v}{G_2}$,
           we have $q \in \dom{G_2}$.
           \\ It is given that $\dom{G'} \disjoint \dom{G_2}$.
           Therefore $q \notin \dom{G_1, G'}$.
           \\ By definition, $\update{(G_1, G')}{q}{v}{(G_2, G')}$.
           \\ Apply Eval-refPlain.

      \ProofCaseRule{Eval-thunkPlain}
           Similar to the Eval-refPlain case.

      \ProofCaseRule{Eval-forcePlain}
         We have $G_1(q) = e_0$.  Therefore $(G_1, G')(q) = e_0$.
         Use the i.h.\ and apply Eval-forcePlain.

      \ProofCaseRule{Eval-getPlain}
         Similar to the Eval-forcePlain case.
  \qedhere
  \end{itemize}
\end{proof}



\subsection{Main result: From-scratch consistency}
\Label{sec:fsc}

At the highest level, the main result (\Theoremref{thm:fsc}) says:

\begin{quote}
\textbf{First approximation} \\
  If $\PreSt{H_1}{p}{w} e !! H_2; t$ by an incremental derivation,
  \\
  then $\PreSt{H_1'}{p}{w} e !! H_2'; t$,
  where $H_1'$ is a non-incremental version of $H_1$
  and $H_2'$ is a non-incremental version of $H_2$.
\end{quote}
%
Using the restriction function from \Sectionref{sec:restriction},
we can refine this statement:

\begin{quote}
\textbf{Second approximation} \\
  If  $\PreSt{H_1}{p}{w} e !! H_2; t$ by an incremental derivation
  and $P_1 \subseteq \dom{H_1}$,
  \\
  then $\PreSt{\restrict{H_1}{P_1}}{p}{w} e !! \restrict{H_2}{P_2}; t$
  by a non-incremental derivation,
  for some $P_2$ such that  $P_1 \subseteq P_2$.
\end{quote}
%
Here, the pointer set $P_1$ gives the scope of the non-incremental
input graph $\restrict{H_1}{P_1}$, and we construct $P_2$
describing the non-incremental output graph
$\restrict{H_2}{P_2}$.

We further refine this statement by involving the derivation's read- and
write-sets: the read set $R$ must be contained in $P_1$, the write set $W$
must be disjoint from $P_1$ (written $\dom{W} \disjoint P_1$), and $P_2$ must be
exactly $P_1$ plus $W$.
In the non-incremental semantics, the store should grow monotonically, so
we will also show $\restrict{H_1}{P_1} \subseteq \restrict{H_2}{P_2}$:

\begin{quote}
\textbf{Third approximation} \\
  If  $\PreSt{H_1}{p}{w} e !! H_2; t$ by an incremental derivation $\D$
  with $\DHasEffects{\D}{R}{W}$,
  \\
  and $P_1 \subseteq \dom{H_1}$
  such that $\dom{R} \subseteq P_1$
  and $\dom{W} \disjoint P_1$
  \\
  then $\PreSt{\restrict{H_1}{P_1}}{p}{w} e !! \restrict{H_2}{P_2}; t$
  \\
  where $\restrict{H_1}{P_1} \subseteq \restrict{H_2}{P_2}$
  and $P_2 = P_1 \cup \dom{W}$.
\end{quote}
%
Even this refinement is not quite enough, because the incremental
system can perform computations in a different order than the non-incremental
system.  Specifically, the Eval-computeDep rule carries out a subcomputation
first, then continues with a larger computation that depends on the subcomputation.
The subcomputation does not fit into the non-incremental derivation at that point;
non-incrementally, the subcomputation is performed when it is demanded by
the larger computation.  Thus, we can't just apply the induction hypothesis on the
subcomputation.

However, the subcomputation is ``saved'' in its (incremental) output graph.
So we incorporate an invariant that all thunks with cached results in the graph
``are consistent'', that is, they satisfy a property similar to the overall consistency
result.  When this is the case, we say that the graph is from-scratch consistent.
The main result, then, will assume that the input graph is from-scratch consistent,
and show that the output graph remains from-scratch consistent.
Since the graph can grow in the interval between the subcomputation of Eval-computeDep
and the point where the subcomputation is demanded, we require that the output
graph $G_2$ of the saved derivation does not contradict the larger, newer graph
$H$.  This is part (4) in the next definition.  (We number the parts from (i) to (ii)
and then from (1) so that they mostly match similar parts in the main result.)

\begin{defn}[From-scratch consistency of a derivation]
\Label{def:fsc}
~\\
  A derivation $\D_i \derives \PreSt{G_1}{p}{w} e !! G_2 ; t$
  is
  \\
  \emph{from-scratch consistent for}
  $P_q \subseteq \dom{G_1}$
  \emph{up to}
  $H$  % ``future'' context
  if and only if
  %
  \begin{enumerate}[(i)]
%  \item % i
%       $[[G1 wf]]$
  \item % ii
       $\D_i \satisfactory$ where $\DHasEffects{\D_i}{R}{W}$
  \item % iii
%     for all $[[P1]]$ such that
     $\dom{R} \subseteq P_q$
     and
     $\dom{W} \disjoint P_q$

      \item[(1)] % 1
           there exists a non-incremental derivation
           $\D_{ni}
            \derives
            \PreSt{\restrict{G_1}{P_q}}{p}{w} e !! \restrict{G_2}{P_2} ; t $

      \item[(2)] % 2
           $\restrict{G_1}{P_q} \subseteq \restrict{G_2}{P_2}$

      \item[(3)] % 3
           $P_2 = P_q \cup \dom{W}$

      \item[(4)] % 4
            $\restrict{G_2}{P_2} \subseteq \restrict{H}{\dom{H}}$
  \end{enumerate}
\end{defn}


\begin{defn}[From-scratch consistency of graphs]
\Label{def:fsc-graph}
~\\
A graph $H$ is
\emph{from-scratch consistent}
\\
if, for all $q \in \dom{H}$ such that $H(q) = (e,t)$,
     \\
     there exists
     $\D_q \derives \PreSt{G_1}{p}{w} e !! G_2 ; t$
     \\
     and
     $P_q \subseteq \dom{G_1}$
     \\
     such that $\D_q$ is from-scratch consistent (\Definitionref{def:fsc})
     for $P_q$ up to $H$.
\end{defn}


The proof of the main result must maintain that the graph is from-scratch
consistent as the graph becomes larger, for which \Lemmaref{lem:fsc-ext-graph}
is useful.

\begin{lem}[Consistent extension]
\Label{lem:fsc-ext}
~\\
  If  $\D_q$ is from-scratch consistent for $P_q$ up to $H$
  \\
  and $H \subseteq H'$
  \\
  then $\D_q$ is from-scratch consistent for $P_q$ up to $H'$.
\end{lem}
\begin{proof}
  Only part (4) of \Definitionref{def:fsc} involves the ``up to'' part
  of from-scratch consistency,
  so we already have (i)--(iii) and (1)--(3).

  We have (4) $\restrict{G_2}{P_2} \subseteq \restrict{H}{\dom{H}}$.
  Using our assumptions, $\restrict{H}{\dom{H}} \subseteq \restrict{H'}{\dom{H'}}$.

  Therefore (4) $\restrict{G_2}{P_2} \subseteq \restrict{H'}{\dom{H'}}$.
\end{proof}


\begin{lem}[Consistent graph extension]
\Label{lem:fsc-ext-graph}
~\\
   If $H$ is from-scratch consistent
   \\
   and $H \subseteq H'$
   \\
   and, for all $q \in \dom{H'} - \dom{H}$ such that $H'(q) = (e,t)$,
   \\
   $~~$  there exists
     $\D_q \derives \PreSt{G_1}{p}{w} e !! G_2 ; t$
     and
     $P_q \subseteq \dom{G_1}$
     \\
     $~~$
     such that $\D_q$ is from-scratch consistent (\Definitionref{def:fsc})
     \\
     $~~$
     for $P_q$ up to $H'$,
   \\
   then
   $H'$ is from-scratch consistent.
\end{lem}
\begin{proof}
  Use \Lemmaref{lem:fsc-ext} on each ``old'' pointer with a cached result in $H$,
  then apply the definitions for each ``new'' pointer with a cached result in
  $\dom{H'} - \dom{H}$.
\end{proof}

At last, we can state and prove the main result, which corresponds to
the ``third approximation'' above, plus the invariant that the graph is
from-scratch consistent (parts (iii) and (4)).

We present most of the proof in a line-by-line style, with the judgment or
proposition being derived in the left column, and its justification in the right column.
In each case, we need to show four different things (1)--(4), some of which are obtained
midway through the case, so we highlight these with ``(1) \Hand'', and so on.

\begin{thm}[From-scratch consistency]
\Label{thm:fsc}
~\\
  Given an incremental $\D_i \derives \PreSt{H_1}{p}{w} e !! H_2 ; t $ where
  \begin{enumerate}[(i)]
%  \item % (i)
%       $[[H1 wf]]$
  \item % (i)
       $\D_i \satisfactory$ where $\DHasEffects{\D}{R}{W}$
  \item % (ii)
     a set of pointers $P_1 \subseteq \dom{H_1}$ is such that $\dom{R} \subseteq P_1$ and $\dom{W} \disjoint P_1$
  \item % (iii)
     $H_1$ is from-scratch consistent (\Definitionref{def:fsc-graph})
%     \\
%     and $[[(restrict Gq' Pq) subseteq (restrict H1 P1)]]$
  \end{enumerate}
  then
  \begin{enumerate}[(1)]
  \item % (1)
    there exists a non-incremental
      $\D_{ni} \derives \PreSt{\restrict{H_1}{P_1}}{p}{w} e !! \restrict{H_2}{P_2} ; t$
  \item % (2)
      $\restrict{H_1}{P_1} \subseteq \restrict{H_2}{P_2}$
  \item % (3)
       $P_2 = P_1 \union \dom{W}$
  \item % (4)
      $H_2$ is from-scratch consistent (\Definitionref{def:fsc-graph}).
  \end{enumerate}
\end{thm}


% Local Variables:
% mode: latex
% TeX-master: "typed-adapton"
% End:


==> meta.tex <==
\section{Metatheory of \calc}
\label{sec:metatheory}

Ideally, we can use well-typedness to discharge certain conditions on the earlier
from-scratch consistency result.  To review, those conditions were:

\begin{itemize}
\item Theorem B.13 precondition (i):

  The evaluation derivation is \emph{globally satisfactory} (Def.\ B.7):
  
  \begin{itemize}
  \item All subderivations are \emph{locally satisfactory} (Def.\ B.6):
    \begin{itemize}
    \item The input graph is well-formed.  Def.\ B.6 (1)
    \item The output graph is well-formed.  Def.\ B.6 (1)
    \item ``$\Dee$ reads $R$ writes $W$'' is defined.  Def.\ B.6 (2)
    \end{itemize}
  \end{itemize}

\item Theorem B.13 precondition (ii):

  Something that relates a set of pointers $P_1$ to $R$ and $W$.

\item Theorem B.13 precondition (iii):

  The input \emph{graph} $H$ is \emph{from-scratch consistent} (Def.\ B.10):

  \begin{itemize}
  \item For all $q \in H$ such that $H(q) = (e, t)$,
    there exists an evaluation derivation $\Dee_e$ of $e$ from $G_1$ to $G_2$ such that
    $\Dee_e$ is from-scratch consistent (B.9) for $P_q$ up to $H$.

    \begin{itemize}
    \item A \emph{derivation} is \emph{from-scratch consistent}
      if \dots

      \begin{itemize}
      \item The derivation is satisfactory (which implies that $R$ and $W$ are defined).  Def.\ B.9 (i)
      \item $P_q$ is properly related to $R$ and $W$.  Def.\ B.9 (ii)
      \item There is a non-incremental derivation\dots ~~Def.\ B.9 (1)
      \item \dots whose graphs are consistent with the incremental graphs.  Def.\ B.9 (2), (3), (4)
      \end{itemize}
    \end{itemize}
  \end{itemize}
\end{itemize}

\begin{conjecture}
~\\
  If
  [$\Gamma$ well-formed]
  \\
  and
  [input graph well-formed]
  \\
  and
  [typing judgment]
  \\
  and
  [evaluation judgment]
  \\
  then
  [globally satisfactory].
\end{conjecture}

Can we also show B.13 (ii) and (iii)?  Do we need to show them?


% Local Variables: 
% mode: latex
% TeX-master: "types"
% End: 



==> mk <==
#!/bin/sh

killall pdflatex
# \rm *.aux
pdflatex fungi-lang
bibtex fungi-lang
pdflatex fungi-lang


==> old-strongnormproof-indextermlang.tex <==
\section{Strong Normalization for Index Terms}
\label{apx:strongnormproof-indexterm}

\begin{lemma}[Substitution]
  \label{lem:subst-index}
  If $\Gamma, a : \sort_a |- i : \sort$
  and $\Gamma |- i_a : \sort_a$
  then $\Gamma |- [i_a/a]i : \sort$.
\end{lemma}
\begin{proof}
  By induction on the derivation of $\Gamma, a : \sort_a |- i : \sort$.
  XXX
\end{proof}

\begin{definition}[$R_{\sort}(e)$]~
        \label{def:strongnormop-index}
        \begin{enumerate}
                  \item $R_{\NmSet}(e)$ iff $e$ halts.
                  \item $R_{(\sort_1 @> \sort_2)}(e)$ if and only if (1) $e$ halts and (2) if $R_{\sort_1}(e')$ then $R_{\sort_2}(e~e')$.
                  \item $R_{\sort_1 ** \sort_2}(e)$ if and only if $e$ halts and $R_{\sort_1}(e)$ and $R_{\sort_2}(e)$.
        \end{enumerate}
\end{definition}

\begin{lemma}[Termination]
        \label{lem:strongnorm-lemma-1-index}
        If $R_{\sort}(e)$ then $e$ halts.
\end{lemma}

\begin{proof}
        By definition of $R_{\sort}(e)$.
\end{proof}

\begin{lemma}[Preservation]
        \label{lem:strongnorm-lemma-2-index}
        If $\Gamma |- e : \sort$ and $\sigma : \Gamma$, then $ |- [\sigma] e : \sort$.
\end{lemma}

\begin{proof}
  By induction on the length of $\sigma$,   using \Lemmaref{lem:subst-index}.
\end{proof}

\begin{lemma}[Normalization]
  \label{lem:strongnorm-lemma-3-index}
  If $\Gamma |- e : \sort$
  and $\sigma : \Gamma$
  then $R_{\sort}([\sigma]e)$.
\end{lemma}

\begin{proof} By induction on the given derivation.

  \begin{itemize}
         \DerivationProofCase{\Sortvar}
                {
                        (a : \sort) \in \Gamma
                }
                {
                        \Gamma |- a : \sort
                }

                \begin{llproof}
                        \Pf{\exists v_i.([\sigma]a}{!!}{v_i)}{By definition of $[\sigma](-)$ XXX ???}
                        \Pf{}{|-}{[\sigma] a : \sort}{By \Lemmaref{lem:strongnorm-lemma-2-index}}
                        \Hand \Pf{}{}{R_{\sort}([\sigma] a)}{Since $[\sigma]a \nteval v_i$ and $|- [\sigma] a : \sort$}
                \end{llproof}

        \DerivationProofCase{\Sortunit}
                {}
                {
                        \Gamma |- \unitindex : \unitsort
                }

                \begin{llproof}
                        \eqPf{[\sigma]\unitindex}{\unitindex}{By definition of $[\sigma](-)$}
                        \Pf{\unitindex}{!!}{\unitindex}{By rule value; Since $\unitindex$ val}
                        \Pf{[\sigma]\unitindex}{!!}{\unitindex}{Since $[\sigma]\unitindex = \unitindex$ and $\unitindex !! \unitindex$}
                        \Pf{\Gamma}{|-}{\unitindex : \unitsort}{Given}
                        \Pf{}{|-}{[\sigma] \unitindex : \unitsort}{By \Lemmaref{lem:strongnorm-lemma-2-index}}
                        \Hand \Pf{}{}{R_{\unitsort}([\sigma] \unitindex)}{Since $[\sigma]\unitindex !! \unitindex$ and $|- [\sigma] \unitindex : \unitsort$}    
                \end{llproof}

        \DerivationProofCase{\Sortpair}
                {
                        \Gamma |- i_1 : \sort_1
                        \\
                        \Gamma |- i_2 : \sort_2
                }
                {
                        \Gamma |- \Pair{i_1}{i_2} : (\sort_1 ** \sort_2)
                }

                \begin{llproof}
                        \Pf{}{}{R_{\sort_1}([\sigma] i_1)}{By inductive hypothesis}
                        \Pf{}{}{R_{\sort_2}([\sigma] i_2)}{By inductive hypothesis}
                        \Pf{\exists v_1.([\sigma] i_1}{!!}{v_1)}{Since $R_{\sort_1}([\sigma] i_1)$}
                        \Pf{\exists v_2.([\sigma] i_2}{!!}{v_2)}{Since $R_{\sort_2}([\sigma] i_2)$}
                        \Pf{([\sigma] i_1, [\sigma] i_2)}{!!}{(v_1, v_2)}{By rule pair}
                        \Pf{[\sigma](i_1, i_2)}{!!}{(v_1, v_2)}{By definition of $[\sigma](-)$}
                        \Pf{}{|-}{[\sigma] (i_1, i_2) : (\sort_1 * \sort_2)}{By \Lemmaref{lem:strongnorm-lemma-2-index}}
                        \Hand \Pf{}{}{R_{(\sort_1 * \sort_2)}([\sigma](i_1\;i_2))}{Since $[\sigma](i_1\;i_2) !! (v_1, v_2)$}\trailingjust{and $~|- [\sigma] (i_1\;i_2) : (\sort_1 ** \sort_2)$}
                \end{llproof}

        \DerivationProofCase{\Sortproj}
                {
                        \Gamma |- i : \sort_1 * \sort_2
                }
                {
                        \Gamma |- \Proj{b}{i} : \sort_b
                }

                \begin{llproof}
                        \Pf{}{}{R_{(\sort_1 * \sort_2)}([\sigma] i)}{By inductive hypothesis}
                        \Pf{}{}{R_{\sort_b}([\sigma] ~\Proj{b}{i})}{By definition of $R_{-}(-)$}
                \end{llproof}

        \DerivationProofCase{\Sortempty}
                {
                        \quad
                }
                {
                        \Gamma |- \emptyset : \namesetsort
                }

        Similar to the \Sortunit case.
      
        \DerivationProofCase{\Sortsingleton}
                {
                        %  \Gamma |- n \wfname
                        \Gamma |- N : \namesort
                }
                {
                        \Gamma |- \{ N \} : \namesetsort
                }

                \begin{llproof}
                        \Pf{[\sigma]\{ N \}}{=}{\{ N \}}{By definition of $[\sigma](-)$}
                        \Pf{}{}{\{ N \} ~\textrm{val}~}{By rule val-singleton}
                        \Pf{\Gamma}{|-}{\{ N \} : \namesetsort}{Given}
                        \Pf{}{|-}{[\sigma] \{ N \} : \namesetsort}{By \Lemmaref{lem:strongnorm-lemma-2-index}}
                        \Hand \Pf{}{}{R_{\namesetsort}([\sigma] \{ N \})}{Since $[\sigma] \{ N \}$ val,$~|- [\sigma] \{ N \} : \namesetsort$}   
                \end{llproof}


        \DerivationProofCase{\Sortunion}
                {
                        \arrayenvbl{
                                \Gamma |- X : \namesetsort
                                \\
                                \Gamma |- Y : \namesetsort
                        }
                }
                {
                        \Gamma |- (X \union Y) : \namesetsort
                }

                \begin{llproof}
                        \Pf{}{}{R_{\namesetsort}([\sigma] X)}{By inductive hypothesis}
                        \Pf{}{}{R_{\namesetsort}([\sigma] Y)}{By inductive hypothesis}
                        \Pf{\exists v_1.([\sigma] X}{!!}{v_1)}{Since $R_{\namesetsort}([\sigma] X)$}
                        \Pf{\exists v_2.([\sigma] Y}{!!}{v_2)}{Since $R_{\namesetsort}([\sigma] Y)$}
                        \Pf{([\sigma] X \union [\sigma] Y)}{!!}{(v_1 \union v_2)}{By rule union}
                        \Pf{[\sigma](X \union Y)}{!!}{(v_1  \union v_2)}{By definition of $[\sigma](-)$}
                        \Pf{}{|-}{[\sigma] (X \union Y) : (\namesetsort)}{By \Lemmaref{lem:strongnorm-lemma-2-index}}
                        \Pf{\xHand}{}{R_{\namesetsort}([\sigma](X \union Y))}{Since $[\sigma](X \union Y) !! (v_1 \union v_2)$}\trailingjust{and $~|- [\sigma] (X \union Y) : \namesetsort$}
                \end{llproof}

        \DerivationProofCase{\Sortsepunion}
                {
                        \arrayenvbl{
                                \Gamma |- X : \namesetsort
                                \\
                                \Gamma |- Y : \namesetsort
                        }
                        \\
                        \extract{\Gamma} ||- X \disj Y : \namesetsort
                }
                {
                        \Gamma |- (X \disj Y) : \namesetsort
                }

                \begin{llproof}
                        \Pf{}{}{R_{\namesetsort}([\sigma] X)}{By inductive hypothesis}
                        \Pf{}{}{R_{\namesetsort}([\sigma] Y)}{By inductive hypothesis}
                        \Pf{\exists v_1.([\sigma] X}{!!}{v_1)}{Since $R_{\namesetsort}([\sigma] X)$}
                        \Pf{\exists v_2.([\sigma] Y}{!!}{v_2)}{Since $R_{\namesetsort}([\sigma] Y)$}
                        \Pf{([\sigma] X \disj [\sigma] Y)}{!!}{(v_1 \disj v_2)}{By rule union}
                        \Pf{[\sigma](X \disj Y)}{!!}{(v_1 \disj v_2)}{By definition of $[\sigma](-)$}
                        \Pf{}{|-}{[\sigma] (X \disj Y) : (\namesetsort)}{By \Lemmaref{lem:strongnorm-lemma-2-index}}
                        \Hand \Pf{}{}{R_{\namesetsort}([\sigma](X \disj Y))}{Since $[\sigma](X \disj Y) !! (v_1 \disj v_2)$}\trailingjust{and $~|- [\sigma] (X \disj Y) : \namesetsort$}
                \end{llproof}


        \DerivationProofCase{\Sortabs}
                {
                        \Gamma, a : \sort_1 |- i : \sort_2
                }
                {
                        \Gamma |- (\Lam{a}{i}) : (\sort_1 @@> \sort_2)
                }
        
                \begin{llproof}
                        \Pf{[\sigma, iii/a]}{|-}{\Gamma'}{Assumption, where $\Gamma' = \Gamma, a : \sort_1$}
                        \Pf{|-}{([\sigma, iii/a](\lam{a} i))} {: (\sort_1 @@> \sort_2)}{By \Lemmaref{lem:strongnorm-lemma-2-index}}
                        \Pf{[\sigma, iii/a] (\lam{a} i)}{=}{(\lam{a} i)}{By definition of $[\sigma](-)$}
\decolumnizePf
                        \Hand \Pf{R_{\sort}([\sigma, iii/a] (\lam{a} i))}{}{}{Since $[\sigma, iii/a](\lam{a} i) !! (\lam{a} i)$} \trailingjust{and $ |- [\sigma, iii/a]  (\lam{a} i) : (\sort_1 @@> \sort_2)$}
            \end{llproof}
          
        \DerivationProofCase{\Sortapply}
                {
                        \Gamma |- i : \sort_1 @@> \sort_2
                        \\
                        \Gamma |- j : \sort_1
                }
                {
                        \Gamma |- i(j) : \sort_2
                }      

                \begin{llproof}
                                \Pf{}{}{R_{(\sort_1 @@> \sort_2)}([\sigma] i)}{By inductive hypothesis}
                                \Pf{}{}{R_{\sort_1}([\sigma] j)}{By inductive hypothesis}
                                \Pf{}{}{R_{\sort_2}(([\sigma]i([\sigma]j)))}{By definition of $R_{-}(-)$}
                                \Hand \Pf{}{}{R_{\sort_2}([\sigma](i(j)))}{By definition of $[\sigma](-)$}
                \end{llproof}

        \DerivationProofCase{\Sortmap}
                {
                        \Gamma |- M : \namesort @> \namesort
                        \\
                        \Gamma |- j : \namesetsort
                }
                {
                        \Gamma |- M[[j]] : \namesetsort
                }

                \begin{llproof}
                        \Pf{}{}{R_{\namesetsort}(j)}{By inductive hypothesis}

                        \Pf{\exists v.(M[[j]]}{!!}{v)}{By \Thmref{thmrefstrongnorm-name}}
                        \Pf{\exists v'.(M[[j]]}{\leadsto}{v)}{By rule Single}
                        \Pf{M[[j]]}{!!}{v'}{By rule map-set}
                        \Pf{|-}{([\sigma](M[[j]])} {: \namesetsort}{By \Lemmaref{lem:strongnorm-lemma-2-index}}
                        \decolumnizePf
                        \Hand \Pf{}{}{R_{\namesetsort}([\sigma](M[[j]])}{Since $M[[j]] =v'$ and $|- ([\sigma](M[[j]]) : \namesetsort$}

%                       \Pf{\exists v.(M[j]}{!!}{v)}{By \Thmref{thmrefstrongnorm-name}}
%                       \Pf{\exists v'.}{(}{\mapset{M}{j} v')}{By rule Single}
%                       \Pf{M[j]}{!!}{v'}{By rule map-set}
%                       \Pf{|-}{([\sigma](M[j])} {: \namesetsort}{By \Lemmaref{lem:strongnorm-lemma-2-index}}
%                       \Hand \Pf{}{}{R_{\namesetsort}([\sigma](M[j])}{Since $M[j] =v'$ and $|- ([\sigma](M[j]) : \namesetsort$}
                \end{llproof}
  \end{itemize}
\end{proof}

\begin{restatable}[Strong Normalization]{theorem}{thmrefstrongnormindex}
        \label{thmrefstrongnorm-index}
        If $\Gamma |- e : \sort$ then $e$ is normalizing.
\end{restatable}

\begin{proof}~\\
        \begin{llproof}
                \Pf{}{}{R_{\sort}(e)}{By \Lemmaref{lem:strongnorm-lemma-3-index}}
                \Hand \Pf{}{}{e ~\textrm{halts}~}{By \Lemmaref{lem:strongnorm-lemma-1-index}}
        \end{llproof}
\end{proof}



% Local Variables:
% mode: latex
% TeX-master: "typed-adapton"
% End:


==> old-table.tex <==
\begin{table}[th]
\def\nope{--}
\def\Yup{\checkmark}
\def\BRK{\\[3pt]}
\newcommand{\LeftColTwo}[2]{%
    \tabularenvr{%
      #1%
      \\
      #2%
      \BRK%
    }%
}
  
  \centering

% correspondence
% mechanism
  \begin{tabular}[t]{r | cccccc}
    \multicolumn{1}{c}{\tabularenvl{
    ~\\
    ~\\
    ~\\
    approach}}
    &
      \tabularenvl{
      ~\\
      ~\\
        general-\\
        purpose
      }
    &
      \tabularenvl{
      ~\\
      ~\\
        general~~~~ \\
        recursion
      }
    &
      \tabularenvl{
         mechanism \\
         to identify \\
         corresponding \\
         subcomputations
%        names
      }
    &
      \tabularenvl{
      ~\\
      ~\\
        detection of \\
          naming errors
      }
    \\ \cmidrule{2-5}
%
%  nope
%    & \nope & \nope & none & \nope
\BRK
    Pramod
    &
\BRK
    DITTO
    &
    no (1a)
\BRK
    \LeftColTwo{
      i3QL
     }{
      \citep{Mitschke14}
     }
    &
      no (2a)
    &
      (2b)
    &
      ?
    &
      ~
\BRK
    % http://www.informatik.uni-marburg.de/~pgiarrusso/ILC/
    \LeftColTwo{
        Incremental $\lambda$-calculus
    }{
        \citep{Cai14}
    }
   &  (3a)
   & \nope     % general recursion
   &  (3b)
\BRK
    AFL
    \citep{Acar02}
    & \Yup & \Yup & no & % n/a    
    \BRK
    \LeftColTwo{
      implicit SAC
    }{
      \citep{Chen11,Chen12}
    }
    & \Yup & \Yup
    & keys (informal)
    & (4a)
\BRK
    \LeftColTwo{
      DeltaML
      \\
      \citep{AcarLeyWild08};
    }{
      CEAL
      \\{}
      \citep{Hammer09}
%      [\citeauthor{Hammer08} \citeyear{Hammer08};
%      \\
%      \citeauthor{Hammer09} \citeyear{Hammer09}, \citeyear{Hammer11};
%      \\
%      \citeauthor{HammerThesis} \citeyear{HammerThesis}%
%      ]
    }
    & \Yup & \Yup
    & keys (informal)
    & (4a) %
      % "sac style"
\BRK
    \LeftColTwo{
      Adapton
    }{
      \citep{Hammer14}
    }
    & \Yup
    & \Yup
    & \tabularenvc{structural \\ (hash-consing)} % informal  % or "structural", or "hash-consing"
    & n/a
\BRK
    \LeftColTwo{
      Nominal Adapton
    }{
      \citep{Hammer15}
    }
    & \Yup & \Yup & names (formal) & dynamic
                             % first-class names
\BRK
    \LeftColTwo{
      Fungi
    }{
      (this paper)
    }
    & \Yup & \Yup & names (formal) & static
                             % first-class names
  \end{tabular}

  \medskip
\raggedright

\runonfontsz{9pt}
    (1a) DITTO is restricted to run-time invariant checking
\\  (2a) i3QL is an incremental query language embedded within Scala
\\  (2b) i3QL's incremental query language supports recursion
\\  (3a) $\lambda$-terms but only tables (multiset-like structures)
\\  (3b) static differentiation implies static det.\ of correspondences
      \\  (TODO: double-check this characterization)
\\  (4a)  % ("hint fail";
      fall back to a global counter and sacrifice stability/reuse now, in the future, or both

  \bigskip

  Reactive Imperative Programming with Dataflow Constraints
  \citep{Demetrescu11}
\\  general purpose: yes.
\\  general recursion: yes (double check).
\\  corresp mechanism: ?
\\  detection: ?
  
  \bigskip
%  https://www.microsoft.com/en-us/research/publication/two-for-the-price-of-one-a-model-for-parallel-and-incremental-computation/
  concurrent revisions
  \citep{Burckhardt11:oopsla}
\\  general purpose: yes.
\\  general recursion: yes (double check).
\\  corresp mechanism: same global call graph position; does not tolerate small edits to the call graph structure without sacrificing stability/reuse.
\\  detection: n/a

  \caption{Comparison of approaches to incremental computation}
  \label{tab:related}
\end{table}


==> pull-abstract <==
#!/bin/sh

# Script to extract the contents of \begin{abstract}...\end{abstract},
# strip newlines (preserving paragraph breaks), remove multiple blank lines,
# remove \emph{} markup,
# remove leading spaces, and remove newlines at end of file.
#
# Usage:
#  pull-abstract
#
# Creates abstract.txt from abstract.tex
#
# sources: various, including http://sed.sourceforge.net/sed1line.txt

if echo a | sed 's_A_X_i' > /dev/null 2>&1 ; then
    # echo sed appears to be GNU sed
    sed=sed
else
    # echo sed is not GNU sed :-/
    # assume that GNU sed is installed as gsed (on OS X, via `brew install gnu-sed`)
    # https://stackoverflow.com/questions/30003570/how-to-use-gnu-sed-on-mac-os-x
    sed=gsed
fi

cat abstract.tex \
  | $sed -e 's/^ *//' \
  | $sed -e 's/\\emph{\([^}]*\)}/\1/g' \
  | $sed -e 's/\\@//g' \
  | $sed -e 's/\~/ /g' \
  | $sed -e 's/\\Fungi/Fungi/g' \
  | $sed -e 's/\$\\lambda\$/lambda/g' \
  | $sed -e 's/\$\\beta\$/beta/g' \
  | $sed -e 's/\$\\eta\$/eta/g' \
  | $sed -e 's/\\"{o}/oe/g' \
  | $sed -e 's/\\"o/oe/g' \
  | $sed -e 's/\\citet{siek15criteria}/Siek et al. (2015)/g' \
  | $sed -e 's/\$\\times\$/x/g' \
  | $sed -e 's/``/"/g' \
  | $sed -e "s/''/\"/g" \
  | $sed -e '1,/begin{abstract}/ d' \
  | $sed -e '/end{abstract}/,$ d' \
  | $sed -e '/^%.*$/ d' \
  | $sed -e 's/%.*$//' \
  | $sed -e 's/^ *$/\$/' \
  | $sed -e ':a;N;$!ba;s/\n/ /g' \
  | $sed -e 's/\$/\n\n/g' \
  | $sed -e 's/^  *//' \
  | $sed -e :a -e '/^\n*$/{$d;N;ba' -e '}' \
  > abstract.txt


==> pull-abstract-html <==
#!/bin/sh

# Script to extract the contents of \begin{abstract}...\end{abstract},
# strip newlines (preserving paragraph breaks), remove multiple blank lines,
# HTMLify \emph{} markup,
# remove leading spaces, and remove newlines at end of file.
#
# Usage:
#  pull-abstract
#
# Creates abstract.html from abstract.tex
#
# sources: various, including http://sed.sourceforge.net/sed1line.txt

if [ "$(uname -s)" == "Darwin" ] # If the system is Mac OS X
then
  sed=gsed
else
  sed=sed
fi

cat abstract.tex \
  | $sed -e 's/^ *//' \
  | $sed -e 's/\\emph{\([^}]*\)}/<i>\1<\/i>/g' \
  | $sed -e 's/\\@//g' \
  | $sed -e 's/\$\\lambda\$/\&lambda;/g' \
  | $sed -e 's/\$\\times\$/\&times;/g' \
  | $sed -e 's/\\Adapton/Adapton/g' \
  | $sed -e 's/\\NominalAdapton/Nominal Adapton/g' \
  | $sed -e 's/\\citet{siek15criteria}/Siek et al. (2015)/g' \
  | $sed -e '1,/begin{abstract}/ d' \
  | $sed -e '/end{abstract}/,$ d' \
  | $sed -e 's/``/\&ldquo;/g' \
  | $sed -e "s/''/\&rdquo;/g" \
  | $sed -e 's/`/\&lsquo;/g' \
  | $sed -e "s/'/\&rsquo;/g" \
  | $sed -e '/^%.*$/ d' \
  | $sed -e 's/%.*$//' \
  | $sed -e 's/^ *$/\$/' \
  | $sed -e ':a;N;$!ba;s/\n/ /g' \
  | $sed -e 's/\$/\n<p>\n/g' \
  | $sed -e 's/^  *//' \
  | $sed -e :a -e '/^\n*$/{$d;N;ba' -e '}' \
  > abstract.html


==> rev-example.tex <==
\newcommand{\Unobserved}{\multicolumn{2}{c|}{\colorbox{lightgray}{\emph{\hphantom{;;}unobserved\hphantom{;;}}}}}
\definecolor{Pink}{rgb}{1.0, 0.80, 0.80}
\newcommand{\Pink}[1]{\colorbox{Pink}{#1}}
%\newcommand{\DeepDeref}[1]{\ensuremath{\keyword{!}^\ast(#1)}}
\newcommand{\InputLabel}[1]{\colorbox{lightshade}{Input:~#1}}

\begin{figure}
  \includegraphics[width=\textwidth]{fig-rev-graph.pdf}
  \caption{Four runs of \code{rev}: two successive runs each of the
    \emph{structural name version} (left hand side, top and bottom),
    and the \emph{explicit name version} (right hand side, top and
    bottom) over a common input list~$[1,2,3,4]$, and input change
    (removal of element~$2$, at position~$b$).
    %%%%%%%%%%%%
    Each thunk for~\code{rev} contains several effect edges:
    %
    to the \code{ref} that it observes (upward),
    %
    to the ref cell that it allocates (downward),
    %
    and to the thunk it allocates and calls as tail-recursive subroutine (rightward).
    \\
    \Tableref{tab:rev} gives further details, listing the arguments
    and results of each call to \code{rev} shown above.
  }
  \label{fig:rev-graph}
\end{figure}


\begin{table}
\begin{tabular}{|ccc|cc|ccc|cc|}
 %----------------------------------------------------------- | ------------------------------------------------------------------
\toprule
  \multicolumn{5}{|c|}{\textbf{Structural}-name version of~\code{rev}} 
& \multicolumn{5}{c|}{\textbf{Explicit}-name version of~\code{rev}}
\\
%----------------------------------------------------------- | ------------------------------------------------------------------
\multicolumn{3}{|c|}{Run 1}
&\multicolumn{2}{c|}{Run 2}
&\multicolumn{3}{c|}{Run 1}
&\multicolumn{2}{c|}{Run 2}
%----------------------------------------------------------- | ------------------------------------------------------------------
\\
\multicolumn{3}{|c|}{\InputLabel{[1,2,3,4]}}
&\multicolumn{2}{c|}{\InputLabel{[1,3,4]}}
&\multicolumn{3}{c|}{\InputLabel{[1,2,3,4]}}
&\multicolumn{2}{c|}{\InputLabel{[1,3,4]}}
%----------------------------------------------------------- | ------------------------------------------------------------------
\\
arg.~\code{l} & arg.~\code{r}       & $\Downarrow$ & arg.~\code{r}        & $\Downarrow$     & 
arg.~\code{l} & arg.~\code{r}       & $\Downarrow$ & arg.~\code{r}        & $\Downarrow$
\\
\midrule
%--- | ----------------------------------------------------- | ------------------------------------------------------------------
%--- | ----------------------------------------------------- | ------------------------------------------------------------------
$a$ & []        & [4,3,2,1]   & []        & [4,3,1]          & $a$   & $z$     & $d'$        & $z$      & $d'$
\\
$b$ & [1]       & [4,3,2,1]   & \Unobserved                  & $b$   & $a'$    & $d'$        &  \Unobserved
\\
$c$ & [2,1]     & [4,3,2,1]   & [1]       & [4,3,1]          & $c$   & $b'$    & $d'$        & \Pink{$a'$}& $d'$
\\
$d$ & [3,2,1]   & [4,3,2,1]   & [3,1]     & [4,3,1]          & $d$   & $c'$    & $d'$        & $c'$     & $d'$
\\
$e$ & [4,3,2,1] & [4,3,2,1]   & [4,3,1]   & [4,3,1]          & $e$   & $d'$    & $d'$        & $d'$     & $d'$
\\
\bottomrule
\end{tabular}
\caption{Four runs of \code{rev}: two successive runs each of the \emph{structural
  name version} (left), and the \emph{explicit name version} (right) over a common
  input list~$[1,2,3,4]$, and input change (removal of element~$2$, at position~$b$).
  \\
%  
  Note that \Figref{fig:rev-graph}'s graph illustration relates the
  input names~($\{a,b,c,d,e\}$), allocated
  pointers~($\{a',b',c',d'\}$) and list contents.  }
\label{tab:rev}
\end{table}


==> strongnormproof-indextermlang.tex <==
\section{Strong Normalization for Name Terms}
\label{apx:strongnormproof-nameterm}


\begin{lemma}[Substitution]
  \label{lem:subst-index}
  If $\Gamma, a : \sort_a |- i : \sort$
  and $\Gamma |- i_a : \sort_a$
  then $\Gamma |- [i_a/a]i : \sort$.
\end{lemma}
\begin{proof}
  By induction on the derivation of $\Gamma, a : \sort_a |- i : \sort$.
  XXX
\end{proof}

\begin{definition}[$R_{\sort}(e)$]~
        \label{def:strongnormop-index}
        \begin{enumerate}
                  \item $R_{\NmSet}(e)$ iff $e$ halts.
                  \item $R_{(\sort_1 @> \sort_2)}(e)$ if and only if (1) $e$ halts and (2) if $R_{\sort_1}(e')$ then $R_{\sort_2}(e~e')$.
                  \item $R_{\sort_1 ** \sort_2}(e)$ if and only if $e$ halts and $R_{\sort_1}(e)$ and $R_{\sort_2}(e)$.
        \end{enumerate}
\end{definition}


We write ``$M$ halts'' when there exists $V$ such that $M \nteval \Mv$.

We write $\sigma : \Gamma$
when, for all $a \in \dom{\Gamma}$, we have $\cdot |- \sigma(a) : \Gamma(a)$.
It follows that $\sigma(a)$ is closed.

\begin{definition}[$R_{\sort}(M)$]
  \label{def:strongnormop-name}
  ~
  \begin{enumerate}
  \item
    $R_{\sort}(M)$ if and only if $\sort \neq (\sort_1 @> \sort_2)$ and $M$ halts.

  \item $R_{(\sort_1 @> \sort_2)}(M)$ if and only if\!
    \tabularenvl{
    (i) $M$ halts and \\
    (ii) for all closed $M'$, if $R_{\sort_1}(M')$ then $R_{\sort_2}(M~M')$.}
  \end{enumerate}
\end{definition}

\begin{lemma}[Substitution]
  \label{lem:subst-name}
  If $\Gamma, a : \sort_a |- M : \sort$
  and $\Gamma |- M_a : \sort_a$
  then $\Gamma |- [M_a/a]M : \sort$.
\end{lemma}
\begin{proof}
  By induction on the derivation of $\Gamma, a : \sort_a |- M : \sort$.
\end{proof}

\begin{lemma}[Closedness]
  \label{lem:closed-name}
  If $M$ is closed
  and $M \nteval \Mv$
  then $\Mv$ is closed.
\end{lemma}
\begin{proof}
  By induction on the derivation of $M \nteval \Mv$.
\end{proof}

\begin{lemma}[Canonical Forms]
  \label{lem:canon-name}
  Suppose $|- \Mv : \sort$.

  \begin{enumerate}
  \item If $\sort = \namesort$ then $\Mv = n$.
  \item If $\sort = (\sort_1 @> \sort_2)$ then $\Mv = (\lam{a} M_0)$
    and $a : \sort_1 |- M_0 : \sort_2$.
  \end{enumerate}
\end{lemma}
\begin{proof}
  By inspection of the given derivation.
\end{proof}

% \begin{lemma}[Termination]
%   \label{lem:strongnorm-lemma-1-name}
%   If $R_{\sort}(M)$ then $M$ halts.
% \end{lemma}
% \begin{proof}
%   By definition of $R_{\sort}(M)$.
% \end{proof}

\begin{lemma}[Multiple Substitution]
  \label{lem:multi-subst-name}
  If $\Gamma |- M : \sort$ and $\sigma : \Gamma$ then $ |- [\sigma]M : \sort$.
\end{lemma}
\begin{proof}
  By induction on the length of $\sigma$, using \Lemmaref{lem:subst-name}.
\end{proof}

\begin{lemma}[Type Preservation]
  \label{lem:type-preservation-name}
  If $|- M : \sort$
  and $M \nteval \Mv$
  then $|- \Mv : \sort$.
\end{lemma}

\begin{lemma}[Preservation]
  \label{lem:preservation-name}
%
  If $R_{\sort}(M)$
  and $M \nteval \Mv$
  then $R_{\sort}(\Mv)$.
\end{lemma}
\begin{proof}
  By induction on $\sort$.

  If $\sort$ does not have the form $(\sort_1 @> \sort_2)$,
  then the only requirement is to show there exists $\Mv'$ such that $\Mv \nteval \Mv'$.
  Let $\Mv' = \Mv$.  Then $\Mv \nteval \Mv'$ by \tevalvalue.

  Otherwise, $\sort = (\sort_1 @> \sort_2)$,
  and we also have to show that for all closed $M_1$
  such that $R_{\sort_1}(M_1)$,
  it is the case that $R_{\sort_2}(M\;M_1)$.

  By definition of $R$, there exists $\Mv_1$ such that $M_1 \nteval \Mv_1$.
  By i.h., $R_{\sort_1}(\Mv_1)$.

  \begin{llproof}
    \Pf{M}{\nteval}{\Mv}  {Above}
    \eqPf{\Mv}{(\lam{a} M_0)}  {By \Lemmaref{lem:canon-name}}
    \Pf{M_1}{\nteval}{\Mv_1}  {Above}
    \Pf{[\Mv_1/a]M_0}{\nteval}{\Mv_2}  {By i.h.}
    \Pf{M\;M_1}{\nteval}{\Mv_2}  {By \tevalapp}
  \end{llproof}
%
%                   \begin{llproof}
%                   \ePf{\Gamma, a : \sort_1}{M : \sort_2}  {Subderivation}
%                   \Pf{}{}{R_{\sort_2}([\sigma_a]M)}  {By i.h.\ with $\sigma_a$ as $\sigma$}
%                   \eqPf{[\sigma_a]M}{[\sigma, M'/a]M = [\sigma][ [\sigma]M'/a]M}{By def.\ of subst.}
%                   \Pf{}{}{R_{\sort_2}([\sigma][ [\sigma]M'/a]M)}  {By above equation}
%                   \Pf{[\sigma_a]M}{\nteval}{\Mv}  {By $R_{\sort_2}([\sigma_a]M)$}
%                   \Pf{[\sigma_a]M'}{\nteval}{\Mv'}  {By $R_{\sort_1}(M')$}
%                   \eqPf{[\sigma_a]M'}{[\sigma]M'} {$a$ not free in $M'$}
%                   \Pf{[\sigma]M'}{\nteval}{\Mv'}  {By above equation}
%                   \proofsep
%                   \Pf{(\lam{a} [\sigma]M_0)}{\nteval}{\lam{a} [\sigma]M_0}  {By \tevalvalue}
%                   \Pf{[\sigma]M'}{\nteval}{\Mv'}  {Above}
%                   \ePf{\Gamma}{\Mv' : \sort_1}  {By \Lemmaref{lem:type-preservation-name}}
%                   \Pf{}{}{R_{\sort_1}([\sigma]\Mv')}  {By i.h.}
%                   \Pf{}{}{R_{\sort_2}([\sigma_a]M_0)}  {By i.h.}
%                   \Pf{[\sigma_a]M_0}{\nteval}{\Mv''} {By definition of $R$}
%                   \eqPf{[\sigma_a]M_0}{[\Mv'/a][\sigma]M_0}  {By def.\ of subst.}
%                   \Pf{[\Mv'/a][\sigma]M_0}{\nteval}{\Mv''} {By above equation}
%                   \Pf{(\lam{a} [\sigma]M_0)\,[\sigma]M'}{\nteval}{\Mv''}  {By \tevalapp}
%                   \Pf{([\sigma]\lam{a} M_0)\,[\sigma]M'}{\nteval}{\Mv''}  {By def.\ of subst.}
%                   \Pf{[\sigma]\big((\lam{a} M_0)\,M'\big)}{\nteval}{\Mv''}  {By def.\ of subst.}
%                   \proofsep
%                 \Hand  \Pf{}{}{R_{\sort_2}\big([\sigma]((\lam{a} M_0) \, M')\big)}  {By definition of $R$}
%                 \end{llproof}
\end{proof}

\begin{lemma}[Normalization]
  \label{lem:norm-name}
  ~\\
  If $\Gamma |- M : \sort$ and $\sigma : \Gamma$
  and, for all $a \in \dom{\Gamma}$, we have $R_{\Gamma(a)}(\sigma(a))$,
  \\
  then $R_{\sort}([\sigma]M)$.
\end{lemma}
\begin{proof} By induction on the derivation of $\Gamma |- M : \sort$.

  \begin{itemize}
%
%                 \begin{llproof}
%                         \eqPf{[\sigma]\unitexp}{\unitexp}{By definition of $[\sigma](-)$}
%                         \Pf{\unitexp}{\nteval}{\unitexp}{By rule \tevalvalue}
%                         \Pf{[\sigma]\unitexp}{\nteval}{\unitexp}{By above equation}
%                         \isavaluePf{\unitexp} {}
%                         \Hand \Pf{}{}{R_{\unitsort}([\sigma]M)} {$[\sigma]M$ halts}
%                 \end{llproof}

        \DerivationProofCase{M-const}
                {}
                {\Gamma |- n : \namesort}

                \begin{llproof}
                        \eqPf{[\sigma]n}{n}{By definition of $[\sigma](-)$}
                        \Pf{n}{\nteval}{n}{By rule \tevalvalue}
                        \Pf{[\sigma]n}{\nteval}{n}{By above equation}
                        \isavaluePf{n} {}
                        \Hand \Pf{}{}{R_{\namesort}([\sigma]M)} {By definition of $R$}
                \end{llproof}

%         \DerivationProofCase{M-unit}
%                 {}
%                 {\Gamma |- \unitexp : \unitsort}
%                 %
%                 Similar to the M-name case.                 

        \DerivationProofCase{M-var}
                {(a : \sort) \in \Gamma}
                {\Gamma |- a : \sort}

                We have $\Gamma(a) = \sort$.
                It is given that $R_{\Gamma(a)}(\sigma(a))$.
                Since $\sigma(a) = [\sigma]a$,
                we have $R_{\sort}{[\sigma]a}$,
                which was to be shown.
%                 \begin{llproof}
% %                        \Pf{\exists v_i.([\sigma]a}{\nteval}{v_i)}{By definition of $[\sigma](-)$}
%                  
%                         \Pf{}{|-}{[\sigma] a : \sort}{From \Lemmaref{lem:multi-subst-name}}
%                         \Hand \Pf{}{}{R_{\sort}([\sigma] a)}{Since $[\sigma]a \nteval v_i$ and $|- [\sigma] a : \sort$}
%                 \end{llproof}

        \DerivationProofCase{M-abs}
                {\Gamma, a : \sort_1 |- M_0 : \sort_2}
                {
                  \Gamma |- (\lam{a} M_0) : (\sort_1 @> \sort_2)
                }

                Suppose that, for some closed $M'$, we have $R_{\sort_1}(M')$.
                By the definition of $R$, that means there exists $\Mv'$
                such that $M' \nteval \Mv'$.
                
                We need to show $R_{\sort_2}\big([\sigma]((\lam{a} M_0) \, M')\big)$.

                Let $\sigma_a = (\sigma, \Mv'/a)$.

                \begin{llproof}
%                  \ePf{\Gamma}{\Mv' : \sort_1}  {By \Lemmaref{lem:type-preservation-name}}
                  \Pf{}{}{R_{\sort_1}(\Mv')}  {By \Lemmaref{lem:preservation-name}}
                  \ePf{\Gamma, a : \sort_1}{M_0 : \sort_2}  {Subderivation}
                  \Pf{}{}{R_{\sort_2}([\sigma_a]M_0)}  {By i.h.\ with $\sigma_a$ as $\sigma$}
%                  \eqPf{[\sigma_a]M_0}{[\sigma, \Mv'/a]M_0 = [\sigma][ [\sigma]\Mv'/a]M_0}{By def.\ of subst.}
%                  \Pf{}{}{R_{\sort_2}([\sigma][ [\sigma]\Mv'/a]M_0)}  {By above equation}
%                  \Pf{[\sigma_a]M_0}{\nteval}{\Mv}  {By $R_{\sort_2}([\sigma_a]M_0)$}
%                  \Pf{[\sigma_a]M'}{\nteval}{\Mv'}  {By $R_{\sort_1}(M')$}
%                  \eqPf{[\sigma_a]M'}{[\sigma]M'} {$a$ not free in $M'$}
%                  \Pf{[\sigma]M'}{\nteval}{\Mv'}  {By above equation}
                  \proofsep
                  \Pf{(\lam{a} [\sigma]M_0)}{\nteval}{\lam{a} [\sigma]M_0}  {By \tevalvalue}
                  \Pf{M'}{\nteval}{\Mv'}  {Above}
%                  \Pf{}{}{R_{\sort_1}([\sigma]\Mv')}  {By i.h.}
%                  \Pf{}{}{R_{\sort_2}([\sigma_a]M_0)}  {By i.h.}
                  \Pf{[\sigma_a]M_0}{\nteval}{\Mv} {By definition of $R$}
                  \eqPf{[\sigma_a]M_0}{[\Mv'/a][\sigma]M_0}  {By def.\ of subst.}
                  \Pf{[\Mv'/a][\sigma]M_0}{\nteval}{\Mv} {By above equation}
                  \Pf{(\lam{a} [\sigma]M_0)\,M'}{\nteval}{\Mv}  {By \tevalapp}
                  \eqPf{M'}{[\sigma]M'}  {$M'$ closed}
                  \Pf{(\lam{a} [\sigma]M_0)\,[\sigma]M'}{\nteval}{\Mv}  {By above equation}
                  \eqPf{(\lam{a} [\sigma]M_0)\,[\sigma]M'}{([\sigma]\lam{a} M_0)\,[\sigma]M'}  {By def.\ of subst.}
                  \continueeqPf{[\sigma]\big((\lam{a} M_0)\,M'\big)} {By def.\ of subst.}
                  \Pf{[\sigma]\big((\lam{a} M_0)\,M'\big)}{\nteval}{\Mv}  {By above equations}
                  \proofsep
                \Hand  \Pf{}{R_{\sort_2}}{\big([\sigma]((\lam{a} M_0) \, M')\big)}  {By definition of $R$}
                \end{llproof}

%                 \begin{llproof}
% %                        \Pf{[\sigma, N/a]}{:}{\Gamma'}{Assumption, where $\Gamma' = (\Gamma, a : \sort_1)$}
% % can't assume the variable is the same! -j.
%                         \Pf{|-}{[\sigma, N/a](\lam{a} M)}{ : (\sort_1 @> \sort_2)}{By \Lemmaref{lem:multi-subst-name}}
%                         \eqPf{[\sigma, N/a] (\lam{a} M)}{(\lam{a} M)}{By definition of $[\sigma](-)$}
%                         \Hand \Pf{R_{\sort}([\sigma, N/a] (\lam{a} M))}{}{}
%                                {Since $[\sigma, N/a](\lam{a} M) \nteval  (\lam{a} M)$}\trailingjust{and $|- [\sigma, N/a]  (\lam{a} M) : (\sort_1 @> \sort_2)$}
%                 \end{llproof}


        \DerivationProofCase{\!M-app}
                {
                        \Gamma |- M_1 : (\sort' @> \sort)
                        \\
                        \Gamma |- M_2 : \sort'
                }
                {\Gamma |- (M_1\;M_2) : \sort}

                \begin{llproof}
                        \Pf{}{}{R_{(\sort' @> \sort)}([\sigma] M_1)}{By i.h.}
                        \Pf{}{}{R_{\sort'}([\sigma] M_2)}{By i.h.}
                        \Pf{}{}{R_{\sort}(([\sigma]M_1)\;[\sigma]M_2)}{By definition of $R$}
                        \Hand \Pf{}{}{R_{\sort}([\sigma](M_1\;M_2))}{By def.\ of subst.}
                \end{llproof}

%         \DerivationProofCase{\!M-pair}
%                 {
%                         \Gamma |- M_1 : \sort_1
%                         \\
%                         \Gamma |- M_2 : \sort_2
%                 }
%                 {\Gamma |- \Pair{M_1}{M_2} : (\sort_1 ** \sort_2)}
%
%                                 \begin{llproof}
%                         \Pf{}{}{R_{\sort_1}([\sigma] M_1)}{By inductive hypothesis}
%                         \Pf{}{}{R_{\sort_2}([\sigma] M_2)}{By inductive hypothesis}
%                         \Pf{\exists v_1.([\sigma] M_1}{\nteval}{v_1)}{Since $R_{\sort_1}([\sigma] M_1)$}
%                         \Pf{\exists v_2.([\sigma] M_2}{\nteval}{v_2)}{Since $R_{\sort_2}([\sigma] M_2)$}
%                         \Pf{([\sigma] M_1, [\sigma] M_2)}{\nteval}{(v_1, v_2)}{By rule \tevaltuple}
%                         \Pf{[\sigma](M_1, M_2)}{\nteval}{(v_1, v_2)}{By definition of $[\sigma](-)$}
%                         \Pf{}{|-}{[\sigma] (M_1, M_2) : (\sort_1 ** \sort_2)}{From \Lemmaref{lem:multi-subst-name}}
%                         \Hand \Pf{}{}{R_{(\sort_1 ** \sort_2)}([\sigma]\Pair{M_1}{M_2})}{Since $[\sigma]\Pair{M_1}{M_2} \nteval (v_1, v_2)$}\trailingjust{and $|- [\sigma] \Pair{M_1}{M_2} : (\sort_1 ** \sort_2)$}
%                 \end{llproof}


        \DerivationProofCase{\!M-bin}
                {
                        \Gamma |- M_1 : \namesort
                        \\
                        \Gamma |- M_2 : \namesort
                }
                {\Gamma |- \NmBin{M_1}{M_2} : \namesort}

                \begin{llproof}
                        \Pf{}{}{R_{\namesort}([\sigma] M_1)}{By i.h.}
                        \Pf{}{}{R_{\namesort}([\sigma] M_2)}{By i.h.}
                        \Pf{[\sigma] M_1}{\nteval}{\Mv_1}{By $R_{\namesort}([\sigma] M_1)$}
                        \ePf{\Gamma}{M_1 : \namesort}  {Subderivation}
                        \ePf{}{[\sigma]M_1 : \namesort}  {By \Lemmaref{lem:multi-subst-name}}
                        \eqPf{\Mv_1}{n_1}  {By \Lemmaref{lem:type-preservation-name}}
                                           \trailingjust{and \Lemmaref{lem:canon-name}}
                        \Pf{[\sigma] M_2}{\nteval}{n_2}{Similar}
                        \Pf{\NmBin{[\sigma] M_1}{[\sigma] M_2}}{\nteval}{\NmBin{n_1}{n_2}}{By rule \tevalbin}
                        \Pf{[\sigma]\NmBin{M_1}{M_2}}{\nteval}{\NmBin{n_1}{n_2}}{By definition of $[\sigma](-)$}
%                        \Pf{}{|-}{[\sigma]\NmBin{M_1}{M_2}: \namesort}{From \Lemmaref{lem:multi-subst-name}}
                        \Hand \Pf{}{}{R_{\namesort}([\sigma]\NmBin{M_1}{M_2})}{By definition of $R$}
                \end{llproof} \qedhere
  \end{itemize}
\end{proof}

\begin{restatable}[Strong Normalization]{theorem}{thmstrongnormname}
        \label{thm:strongnorm-name}
        If $|- M : \sort$ then there exists $\Mv$ such that $M \nteval \Mv$.
\end{restatable}
\begin{proof}
  By \Lemmaref{lem:norm-name}, $R_{\sort}(M)$.

  By definition of $R$, there exists $\Mv$ such that $M  \nteval \Mv$.
\end{proof}



% Local Variables: 
% mode: latex
% TeX-master: "typed-adapton"
% End: 


==> table.tex <==
\begin{table}[th]
\def\nope{--}
\def\Yup{\checkmark}
\def\BRK{\\[3pt]}
\newcommand{\LeftColTwo}[2]{%
    \tabularenvr{%
      #1%
      \\
      #2%
      \BRK%
    }%
}
  
\centering

% correspondence
% mechanism
  \runonfontsz{9pt}
  \begin{tabular}[t]{r | cccccc}
    \multicolumn{1}{c}{\tabularenvl{
    ~\\
    ~\\
    ~\\
    approach}}
    &
      \tabularenvl{
      ~\\
      ~\\
        general-\\
        purpose
      }
    &
      \tabularenvl{
      ~\\
      ~\\
        general~~~~ \\
        recursion
      }
    &
      \tabularenvl{
         mechanism \\
         to identify \\
         corresponding \\
         subcomputations
%        names
      }
    &
      \tabularenvl{
      ~\\
      ~\\
        detection of \\
          naming errors
      }
    \\ \cmidrule{2-5}
%
%  nope
%    & \nope & \nope & none & \nope
\BRK
    Pramod
    &
\BRK
    DITTO \citep{Shankar07}
    &
    no (1a)
\BRK
      i3QL
      \citep{Mitschke14}
    &
      no (2a)
    &
      (2b)
    &
      ?
    &
      ~
\BRK
    % http://www.informatik.uni-marburg.de/~pgiarrusso/ILC/
    \LeftColTwo{
        Incremental $\lambda$-calculus
    }{
        \citep{Cai14}
    }
   &  (3a)
   & \nope     % general recursion
   &  (3b)
\BRK
    AFL
    \citep{Acar02}
    & \Yup & \Yup & no & % n/a    
    \BRK
      implicit SAC \citep{Chen11,Chen12}
    & \Yup & \Yup
    & keys (informal)
    & (4a)
\BRK
    \LeftColTwo{
      DeltaML \citep{AcarLeyWild08};
    }{
      CEAL \citep{Hammer09}
%      [\citeauthor{Hammer08} \citeyear{Hammer08};
%      \\
%      \citeauthor{Hammer09} \citeyear{Hammer09}, \citeyear{Hammer11};
%      \\
%      \citeauthor{HammerThesis} \citeyear{HammerThesis}%
%      ]
    }
    & \Yup & \Yup
    & keys (informal)
    & (4a) %
      % "sac style"
\BRK
%    \LeftColTwo{
      Adapton
%    }{
      \citep{Hammer14}
%    }
    & \Yup
    & \Yup
    & \tabularenvc{structural \\ (hash-consing) \vspace*{0.8ex}} % informal  % or "structural", or "hash-consing"
    & n/a
\BRK
    \LeftColTwo{
      Nominal Adapton
    }{
      \citep{Hammer15}
    }
    & \Yup & \Yup & names (formal) & dynamic
                             % first-class names
\BRK
%    \LeftColTwo{
      Fungi
%    }{
      (this paper)
%    }
    & \Yup & \Yup & names (formal) & static
                             % first-class names
  \end{tabular}

  \medskip
\raggedright

\runonfontsz{9pt}
    (1a) DITTO is restricted to run-time invariant checking
\\  (2a) i3QL is an incremental query language embedded within Scala
\\  (2b) i3QL's incremental query language supports recursion
\\  (3a) $\lambda$-terms but only tables (multiset-like structures)
\\  (3b) static differentiation implies static det.\ of correspondences
      \\  (TODO: double-check this characterization)
\\  (4a)  % ("hint fail";
      fall back to a global counter and sacrifice stability/reuse now, in the future, or both

  \bigskip

%  Reactive Imperative Programming with Dataflow Constraints
  
  \citep{Demetrescu11}
\\  general purpose: yes.
\\  general recursion: yes (double check).
\\  corresp mechanism: ?
\\  detection: ?
  
  \bigskip
%  https://www.microsoft.com/en-us/research/publication/two-for-the-price-of-one-a-model-for-parallel-and-incremental-computation/
  concurrent revisions
  \citep{Burckhardt11:oopsla}
\\  general purpose: yes.
\\  general recursion: yes (double check).
\\  corresp mechanism: same global call graph position; does not tolerate small edits to the call graph structure without sacrificing stability/reuse.
\\  detection: n/a

  \caption{Comparison of approaches to incremental computation}
  \label{tab:related}
\end{table}


% Local Variables: 
% mode: latex
% TeX-master: "fungi-lang"
% End: 

